Optimal qubit circuits for quantum-enhanced telescopes

We propose two optimal phase-estimation schemes that can be used for quantum-enhanced long-baseline interferometry. By using distributed entanglement, it is possible to eliminate the loss of stellar photons during transmission over the baselines. The first protocol is a sequence of gates using nonlinear optical elements, optimized over all possible measurement schemes to saturate the Cram\'er-Rao bound. The second approach builds on an existing protocol, which encodes the time of arrival of the stellar photon into a quantum memory. Our modified version reduces both the number of ancilla qubits and the number of gate operations by a factor of two.

==> FI_section_backup.tex <==
To quantify and compare the information obtained by specific measurement schemes, we use the Fisher information~\cite{Tsang2011}
\begin{equation} \label{eq:fisher}
    f = \sum_{k} \frac{1}{p_k} \left( \frac{\partial p_k}{\partial \Phi} \right)^2,
\end{equation}
where $p_k$ is the probability of obtaining measurement outcome $k$. The variance of the phase estimator is bounded by the inverse of the Fisher information, $\Delta\Phi^2\geq 1/f$, so a measurement scheme with higher Fisher information is able to provide better resolution.

The maximum possible Fisher information of a quantum measurement on the stellar photon state \eqref{eq:psi-star}, 
optimized over all possible measurement schemes, is given by the quantum Fisher information (QFI)~\cite{Paris2008}. The QFI is given by
\begin{equation}
    f(\Phi) \leq h(\Phi) = \text{Tr}\left[ \rho_\text{star} L_\Phi L_\Phi \right]=1,
\end{equation}
where $\rho_\text{star}$ is the density matrix representing the state of the star photon and $L_\Phi$ is the symmetric logarithmic derivative, defined by
\begin{equation} \label{eq:SLD_def}
    \frac{L_\Phi \rho_\text{star} + \rho_\text{star} L_\Phi}{2} = \frac{\partial \rho_\text{star}}{\partial \Phi},
\end{equation}
which for the state \eqref{eq:psi-star} (conditioned on the arrival of a photon) is satisfied by
\begin{equation}
    L_\Phi = i
    \begin{pmatrix}
        0 & -e^{-i\Phi} \\
        e^{i\Phi} & 0 
    \end{pmatrix}.
\end{equation}
We define any protocol whose Fisher information saturates the QFI, $f(\Phi)=h(\Phi)$, as an optimal measurement scheme. The Gottesman et al. protocol presented in \cite{Gottesman2012} has a Fisher information of $f=h/2$, so although it has certain advantages over classical interferometry, it is not an optimal measurement scheme. This result reflects the fact that only half of the star photons are used for the estimation of the visibility, because half the time both photons arrive at the same telescope, and those cases are discarded. We propose a protocol that uses all the star photons, and thus gives twice the precision in the estimate of $\Phi$. 
